Life after BERT: What do Other Muppets Understand about Language?

Existing pre-trained transformer analysis works usually focus only on one or two model families at a time, overlooking the variability of the architecture and pre-training objectives. In our work, we utilize the oLMpics benchmark and psycholinguistic probing datasets for a diverse set of 29 models including T5, BART, and ALBERT. Additionally, we adapt the oLMpics zero-shot setup for autoregressive models and evaluate GPT networks of different sizes. Our findings show that none of these models can resolve compositional questions in a zero-shot fashion, suggesting that this skill is not learnable using existing pre-training objectives. Furthermore, we find that global model decisions such as architecture, directionality, size of the dataset, and pre-training objective are not predictive of a model's linguistic capabilities.

==> ACL/Archive/Table3_Zero-Shot.tex <==
\begin{table*}
\centering
\footnotesize
\begin{tabular}{ l | c c c c c c c c}
\toprule
& \thead{Age \\  Comp.} & \thead{Always \\  Never} & \thead{Object \\ Comp.} & \thead{Antonym \\ Negation} & \thead{Taxonomy \\ Conj.} & \thead{Multi-hop \\ Comp.} \\
\midrule
        Majority vote & 50.6 & 36.1 & 50.6 & 50.2 & 34.0 & 34.0 \\
        \midrule
        $\mathrm{BERT}_\mathrm{base}$ & 49.4 & 13.3 & 55.4 & 53.8 & 46.7 & 33.2 \\ 
        $\mathrm{BERT}_\mathrm{large}$ & 50.6 & 22.5 & 52.4 & 51.0 & \textbf{53.9} & 33.8 \\ 
        $\mathrm{BERT}_\mathrm{large}$ WWM & 76.6 & 10.7 & 55.6 & 57.2 & 46.2 & 33.8 \\ 
        $\mathrm{RoBERTa}_\mathrm{large}$ & 98.6 & 13.5 & 87.4 & \textbf{74.4} & 45.4 & 28.0 \\ 
        \midrule
        $\mathrm{DistilBERT}_\mathrm{base}$ & 49.4 & 15.0 & 50.8 & 50.8 & 46.9 & 33.4 \\ 
        $\mathrm{AlBERT}_\mathrm{base}$ & 47.0 & 23.2 & 50.6 & 52.6 & - & 34.0 \\ 
        $\mathrm{AlBERT}_\mathrm{large}$ & 52.8 & 30.7 & 49.2 & 50.2 & - & 34.0 \\ 
        $\mathrm{AlBERT}_\mathrm{xlarge}$ & 39.8 & 26.1 & 50.4 & 44.6 & - & 32.2 \\ 
        $\mathrm{AlBERT}_\mathrm{xxlarge}$ & 95.4 & 22.9 & 61.0 & 66.4 & - & 34.0 \\ 
        $\mathrm{AlBERTv2}_\mathrm{base}$ & 50.6 & 21.4 & 49.4 & 54.2 & - & 34.0 \\ 
        $\mathrm{AlBERTv2}_\mathrm{large}$ & 51.4 & 31.7 & 50.6 & 55.2 & - & 34.0 \\ 
        $\mathrm{AlBERTv2}_\mathrm{xlarge}$ & 46.2 & \textbf{37.9} & 50.6 & 62.4 & - & 32.4 \\ 
        $\mathrm{AlBERTv2}_\mathrm{xxlarge}$ & 93.8 & 23.9 & 78.8 & 64.8 & - & 34.0 \\ 
        $\mathrm{BART}_\mathrm{large}$ & 49.4 & 14.3 & 50.8 & 53.8 & 42.6 & 33.8 \\ 
        $\mathrm{T5}_\mathrm{small}$ & 49.4 & 16.1 & 48.2 & 47.0 & 49.3 & 33.8 \\ 
        $\mathrm{T5}_\mathrm{base}$ & 49.4 & 10.7 & 59.0 & 53.4 & 46.6 & 33.6 \\ 
        $\mathrm{T5}_\mathrm{large}$ & 94.0 & 25.7 & 79.8 & 59.2 & 42.2 & 33.8 \\ 
        $\mathrm{T5}_\mathrm{xl}$ & \textbf{100.0} & 20.4 & \textbf{90.0} & 68.4 & 41.2 & 34.4 \\ 
        $\mathrm{T5v1.1}_\mathrm{small}$ & 49.4 & 34.3 & 50.6 & 51.4 & 48.2 & \textbf{37.8} \\ 
        $\mathrm{T5v1.1}_\mathrm{base}$ & 50.6 & 11.8 & 56.0 & 45.0 & 49.9 & 37.6 \\ 
        $\mathrm{T5v1.1}_\mathrm{large}$ & 49.6 & 15.7 & 50.6 & 47 & 41.7 & 33.8 \\ 
        $\mathrm{T5v1.1}_\mathrm{xl}$ & 49.4 & 23.9 & 49.4 & 54.2 & \textbf{53.9} & 33.8 \\ 
        $\mathrm{UniLM}_\mathrm{base}$ & 47.9 & 15.5 & 47.8 & 43.5 & 45.1 & 34.9 \\ 
        $\mathrm{UniLM}_\mathrm{large}$ & 47.9 & 19.2 & 61.1 & 50.8 & 50.2 & 33.1 \\
        $\mathrm{GPT2}_\mathrm{base-0.1B}$ & 47.6 & 9.0 & 50.3 & 53.3 &  49.1 & 32.6 \\
        $\mathrm{GPT2}_\mathrm{medium-0.3B}$ & 50.1 & \underline{31.3} & 50.3 & 52.8 & 51.9 & 34.0 \\ 
        $\mathrm{GPT2}_\mathrm{large-0.8B}$ & 69.6 & 26.0 & 50.5 & 59.0 &  46.9 & 34.0 \\ 
        $\mathrm{GPT}_\mathrm{NEO-1.3B}$ & 58.6 & 29.0 & 52.1 & 65.2 & 50.6 & 33.3 \\
        $\mathrm{GPT2}_\mathrm{xl-1.5B}$ & 51.9 & 26.6 & 52.6 & 60.6 & 45.8 & 34.0 \\
        \bottomrule
\end{tabular}
\caption{Zero-shot oLMpics evaluation on MC-MLM tasks. Majority vote here is the accuracy when predicting the most frequent class. The first 4 models are our reproduction of the original oLMpics results.
The best result on each task is highlighted in bold.
Confidence intervals estimated via bootstrapping 20\% of the data, show errors about 1-2 absolute points.
}
\label{tab:mc-mlm-zero-shot}
\end{table*}

==> ACL/Archive/Table4_antonym_negation_prompts.tex <==
\begin{table*}
\toprule
% \centering
\begin{tabular}{p{4.25cm} | p{6.25cm} | c c c} 
% \begin{tabular}{l | l | c c c} 
\label{tab:prompts-antonym-negation}
Prompt & Input sequence(example) & GPT2 & GPT2-m & GPT2-l\\
\midrule
     oLMpics  & It was really/not sane, it was really insane & 53.3 & 52.8 & 59.0 \\
\midrule
     C\~AB  & It was really insane. Was it sane ?  & 51.6 & \textbf{58.2} & \textbf{55.6} \\
     C\~A+'really'+B & It was really insane. Was it really sane ? & 50.2 & 54 & 50.2 \\
     AB+'entails'+C & It was sane entails it was really insane ? & 49.8 & 50.2 & 50 \\
     'Sentence 1:'+AB+'Sentence 2'+C. Is Sentence 1 synonym of Sentence 2?' & Sentence 1: "It was sane. Sentence 2:  It was really insane. Is Sentence 1   synonym of Sentence 2 ?  & \textbf{59.6} & 50.2 & 46.8 \\
\bottomrule
\end{tabular}
\caption{Evaluation on reformatted Antonym Negation task. Ramdom baseline accuarcy is 50\%. Original input sequence: "It was [MASK] sane , it was really insane.".  A:"It was", B:"sane", C:"it was really insane", \~A : 'was It'. m : medium, l:large.}
\label{tab:reformatted-gpt2}
\end{table*}


==> ACL/t5_head_specialization.tex <==
% Moved to https://www.overleaf.com/5181385451hnhqgxstzvvz
